Observation of muonic Dalitz decays of $\chi_{b}$ mesons and precise spectroscopy of hidden-beauty states

The decays of the $\chi_{b1}(1P)$, $\chi_{b2}(1P)$, $\chi_{b1}(2P)$ and $\chi_{b2}(2P)$ mesons into the $\Upsilon(1S)\mu^+\mu^-$ final state are observed with a high significance using proton-proton collision data collected with the LHCb detector and corresponding to an integrated luminosity of 9fb$^{-1}$. The newly observed decays together with the $\Upsilon(2S)\rightarrow \Upsilon(1S)\pi^+\pi^-$ and $\Upsilon(3S)\rightarrow \Upsilon(2S)\pi^+\pi^-$ decay modes are used for precision measurements of the mass and mass splittings for the hidden-beauty states.

==> Authorship_LHCb-PAPER-2024-025-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
Z. Aliouche,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
P. Andreola,
M. Andreotti,
D. Andreou,
A. Anelli,
D. Ao,
F. Archilli,
M. Argenton,
S. Arguedas Cuendis,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ataíde Da Silva,
M. Atzeni,
B. Audurier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
M. Bartolini,
J. Bartz,
J.M. Basels,
S. Bashir,
G. Bassi,
B. Batsukh,
P. B.  Battista,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. B.  Behling,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
C. Betancourt,
F. Betti,
J.  Bex,
Ia. Bezshyiko,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
A. Brossa Gonzalo,
J. Brown,
D. Brundu,
E. Buchanan,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
A. C.  Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
S. Cali,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
J. Castro Godinez,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
D. Cervenkov,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
M. Chefdeville,
C. Chen,
S. Chen,
Z. Chen,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
M. C.  Colonna,
A. Comerma-Montells,
L. Congedo,
A. Contu,
N. Cooke,
I. Corredoira ,
A. Correia,
G. Corti,
J.J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
A. Danilina,
P. d'Argent,
A.  Davidson,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
V. Dedu,
S.  Dekkers,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
W. Duan,
P. Duda,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
J. Ellbracht,
S. Ely,
A. Ene,
E. Epple,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
L.N. Falcao,
Y. Fan,
B. Fang,
L. Fantini,
M. Faria,
K.   Farmer,
D. Fazzini,
L. Felkowski,
M. Feng,
M. Feo,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
L. F.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
Y. Fujii,
T. Fulghesu,
E. Gabriel,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
K. G.  Garg,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. G.  Ghizzo,
Z. Ghorbanimoghaddam,
L. Giambastiani,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
P. Gironella Gironell,
C. Giugliano,
M.A. Giza,
E.L. Gkougkousis,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
M. Guittiere,
V. Guliaeva,
P. A. G{\"u}nther,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
J. Haimberger,
M. Hajheidari,
G. H.  Hallett,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
M. Hartmann,
S. Hashmi,
J. He,
F. Hemmer,
C. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Hicheur,
G. Hijano Mendizabal,
D. Hill,
S.E. Hollitt,
J. Horswill,
R. Hou,
Y. Hou,
N. Howarth,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
T.P. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
D. Karpenkov,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O.K. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
B. K.  Kutsenko,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. Lesser,
B. Leverington,
A. Li,
C.  Li,
H. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q.  Li,
S. Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Z. Lian,
X. Liang,
S. Libralon,
C. Lin,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
A. Lobo Salvia,
A. Loi,
J. Lomba Castro,
T. Long,
J.H. Lopes,
A. Lopez Huertas,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
A. Maevskiy,
D. Magdalinski,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
A. Modak,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
S. Okamura,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
M. Olocco,
C.J.G. Onderwater,
R.H. O'Neil,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
B. Passalacqua,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
A. Pereiro Castro,
P. Perret,
A. Perro,
K. Petridis,
A. Petrolini,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
G. Punzi,
S.  Qasim,
Q. Q.  Qian,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
R.I. Rabadan Trejo,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
R. Ribatti,
G. R.  Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
R. Sadek,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
S. Schulte,
M.H. Schune,
R. Schwemmer,
G. Schwering,
B. Sciascia,
A. Sciuccati,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
E. Smith,
K. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
E.N. Stein,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
D. Sundfeld,
W. Sutcliffe,
P.N. Swallow,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
M.D. Tat,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
D.  Vico Benet,
P. V.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
G. Vouters,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
C. Wang,
G. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.R.J. Williams,
R. Williams,
Z.  Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
D. Yang,
K.  Yang,
S. Yang,
X. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Z.  Zhang,
Y. Zhao,
A. Zharkova,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)


